Simplifying Graph Convolutional Networks

Graph Convolutional Networks (GCNs) and their variants have experienced significant attention and have become the de facto methods for learning graph representations. GCNs derive inspiration primarily from recent deep learning approaches, and as a result, may inherit unnecessary complexity and redundant computation. In this paper, we reduce this excess complexity through successively removing nonlinearities and collapsing weight matrices between consecutive layers. We theoretically analyze the resulting linear model and show that it corresponds to a fixed low-pass filter followed by a linear classifier. Notably, our experimental evaluation demonstrates that these simplifications do not negatively impact accuracy in many downstream applications. Moreover, the resulting model scales to larger datasets, is naturally interpretable, and yields up to two orders of magnitude speedup over FastGCN.

==> figures/analogy.tex <==
% \begin{figure}[t]
% \centering
% \small
% \begin{tikzpicture}[node distance=1.4cm, every node/.style={fill=white}, align=center, scale=0.7]
%   \tikzset{ % Specifications for style of nodes:
%       head/.style = {minimum width=1cm, minimum height=1cm, text centered},
%       base/.style = {rectangle, rounded corners, draw=black, minimum width=2.6cm, minimum height=1cm, text centered},
%       perceptron/.style = {base, fill=color_perceptron},
%       mlp/.style = {base, fill=color_mlp},
%       filter/.style = {base, fill=color_filter},
%       cnn/.style = {base, fill=color_cnn},
%       gcn/.style = {base, fill=color_gcn},
%       sgr/.style = {base, fill=color_sgr},
%   }
%   \node (linear) [head] {\textbf{Linear}};
%   \node (nonlinear) [head, right of=linear, xshift=2.0cm] {\textbf{Nonlinear}};
%   \node (perceptron) [perceptron, below of=linear, yshift=0.4cm] {Perceptron \\ \citep{rosenblatt1958perceptron}};
%   \node (mlp) [mlp, right of=perceptron, xshift=2.0cm] {MLP \\ \citep{rosenblatt1961principles}};
%   \node (filter) [filter, below of=perceptron] {Predefined Filters \\ \citep{sobel19683x3}};
%   \node (cnn) [cnn, below of=mlp] {CNN \\ \citep{lecun1989backpropagation}};
%   \node (sgr) [sgr, below of=filter] {\large \textbf{?}};
%   \node (gcn) [gcn, below of=cnn] {GCN \\ \citep{gcn}};
  
%   \node (input) [head, left of=linear, xshift=-1.2cm] {\textbf{Domain}};
%   \node (entity) [head, below of=input, yshift=0.4cm] {No \\ Structure};
%   \node (image) [head, below of=entity] {Regular \\ grids};
%   \node (graph) [head, below of=image] {Irregular \\ graphs};
  
% %   \draw[color_mlp,thick,dotted] ($(entity.north west)+(-0.2,0.2y)$)  rectangle ($(mlp.south east)+(0.2,-0.2)$);
% %   \draw[color_cnn,thick,dotted] ($(image.north west)+(-0.2,0.2y)$)  rectangle ($(cnn.south east)+(0.2,-0.2)$);
% %   \draw[color_gcn,thick,dotted] ($(graph.north west)+(-0.2,0.2y)$)  rectangle ($(gcn.south east)+(0.2,-0.2)$);
% \end{tikzpicture}
% \caption{The shallow and linear version of GCN has not been thoroughly studied yet.} \label{fig:analogy}
% \end{figure}

\begin{figure}[t]
\centering
\small
\begin{tikzpicture}[node distance=1.4cm, every node/.style={fill=white}, align=center, scale=0.7]
  \tikzset{ % Specifications for style of nodes:
      head/.style = {minimum width=1cm, minimum height=1cm, text centered},
      base/.style = {rectangle, rounded corners, draw=black, minimum width=2.6cm, minimum height=1cm, text centered},
      perceptron/.style = {base, fill=color_perceptron},
      mlp/.style = {base, fill=color_mlp},
      filter/.style = {base, fill=color_filter},
      cnn/.style = {base, fill=color_cnn},
      gcn/.style = {base, fill=color_gcn},
      sgr/.style = {base, fill=color_sgr},
  }
  \node (linear) [head] {\textbf{Linear}};
  \node (nonlinear) [head, right of=linear, xshift=2.0cm] {\textbf{Nonlinear}};
  \node (perceptron) [perceptron, below of=linear, yshift=0.4cm] {Perceptron\\(1958)};
  \node (mlp) [mlp, right of=perceptron, xshift=2.0cm] {MLP\\(1961)};
  \node (filter) [filter, below of=perceptron] {Predefined Filters\\(1968)};
  \node (cnn) [cnn, below of=mlp] {CNN\\(1989)};
  \node (sgr) [sgr, below of=filter] {\large \textbf{?}};
  \node (gcn) [gcn, below of=cnn] {GCN\\(2016)};
  
  \node (input) [head, left of=linear, xshift=-1.2cm] {\textbf{Domain}};
  \node (entity) [head, below of=input, yshift=0.4cm] {No \\ Structure};
  \node (image) [head, below of=entity] {Regular \\ grids};
  \node (graph) [head, below of=image] {General \\ graphs};
  
%   \draw[color_mlp,thick,dotted] ($(entity.north west)+(-0.2,0.2y)$)  rectangle ($(mlp.south east)+(0.2,-0.2)$);
%   \draw[color_cnn,thick,dotted] ($(image.north west)+(-0.2,0.2y)$)  rectangle ($(cnn.south east)+(0.2,-0.2)$);
%   \draw[color_gcn,thick,dotted] ($(graph.north west)+(-0.2,0.2y)$)  rectangle ($(gcn.south east)+(0.2,-0.2)$);
\end{tikzpicture}
\caption{The shallow and linear version of GCN has not been thoroughly studied yet.} \label{fig:analogy}
\end{figure}
